Training Deep Neural Networks via Direct Loss Minimization

Supervised training of deep neural nets typically relies on minimizing cross-entropy. However, in many domains, we are interested in performing well on metrics specific to the application. In this paper we propose a direct loss minimization approach to train deep neural networks, which provably minimizes the application-specific loss function. This is often non-trivial, since these functions are neither smooth nor decomposable and thus are not amenable to optimization with standard gradient-based methods. We demonstrate the effectiveness of our approach in the context of maximizing average precision for ranking problems. Towards this goal, we develop a novel dynamic programming algorithm that can efficiently compute the weight updates. Our approach proves superior to a variety of baselines in the context of action classification and object detection, especially in the presence of label noise.

==> relate.tex <==
\section{Related work}

%{\color{red} add in this section Rich work, and others that were before in the intro, note that I have just commented it}

%Task loss decomposable
The task-loss, just like the target distribution, is an important component during training of classification and ranking algorithms. Early work has focused on using decomposable metrics such as the 0-1 loss, because it was also the metric of choice when reporting results. However, in recent years, typical evaluation metrics have become more and more refined. Examples for currently employed evaluation metrics are average precision (AP) or normalized discounted cumulative gain.

%Task loss non-decomposable
None of the aforementioned more complex evaluation metrics is decomposable and therefore as easy to evaluate as the 0-1 error. It is hence common to employ the 0-1 error metric during training of a classifier, while reporting results using the more appropriate measures. However the 0-1 error is at best highly correlated with the desired metric. Finding efficient techniques to include the metric of choice into the optimization is therefore desirable. For a series of task-loss functions \citet{TarlowAISTATS2012} derive efficient optimization techniques. Similarly, \citet{yue2007support,mohapatra2014efficient} propose efficient methods to incorporate AP into learning algorithms. Along their line of work we propose a general dynamic programming based algorithm to efficiently optimize for the AP task loss. Our extension is necessary for direct loss minimization because ...

%Surrogate losses
Importantly, task-loss functions for labeling or ranking tasks are discrete and hence hard to optimize directly. Surrogates which provide a smooth and continuous approximation for the task-loss are therefore common. Among the most popular surrogates are the log-loss which corresponds to optimizing the cross-entropy, and the hinge-loss.
Less popular but none-the-less important are non-convex approximations such as the ramp-loss~\citep{CollobertICML2006} and other constructions obtained by introducing distributions
as illustrated by~\citet{VolkovsICML2009}.

All those surrogates approximate the desired task-loss and are, again, at best correlated.
In recent years, direct loss minimization for linear scoring functions~\citep{hazan2010direct} has been demonstrated to yield encouraging results.
For example,~\citet{hazan2010direct} used the technique for phoneme-to-speech alignment on the TIMIT dataset optimizing the \textit{$\tau$-alignment loss} and the \textit{$\tau$-insensitive loss}.
\cite{KeshetInterspeech2011} illustrated applicability of the method to hidden Markov models for speech.
Direct loss minimization was also shown to work well for inverse optimal control by \cite{doerr2015direct}. %Policy Search on a reward function

In contrast to all the aforementioned methods for direct loss minimization, in this paper we tackled the case where the scoring function is non-linear and also not necessarily convex with respect to model parameters. In addition we illustrated its applicability for non-decomposable loss functions.

%Moreover, in all the aforementioned cases, loss-augmented inference is typically performed quickly because the task-loss decomposes in a way similar to the scoring function.
%In contrast, in this paper we additionally illustrate that direct loss minimization can still be applied beneficially even if the task-loss is not decomposable. We demonstrate this by extending an efficient technique for minimization of the average precision (AP) loss metric~\citep{yue2007support,mohapatra2014efficient}.

%Hence, in this paper, we illustrate how to perform direct task-loss minimization for not decomposable loss functions such as the AP loss which admit an efficient search.
%Related to the work presented in this paper are methods that design efficient techniques for loss-augmented inference based optimization occurring in hinge-loss surrogate functions, \eg, message passing methods by~\citet{TarlowAISTATS2012}. Construction of surrogates other than hinge-loss or log-loss, as illustrated by~\citet{VolkovsICML2009}, are equally related.

%In contrast, our goal in this paper is to \emph{directly} optimize the non-decomposable AP task-loss to train a deep neural network as our scoring function. %The presented approach can also be applied in combination with deep structured distributions~\citep{JaderbergICLR2015,ZhengARXIV2015,SchwingARXIV2015,ChenSchwingICML2015}.
%No surrogate like the hinge- or log-loss is involved. %This requires us to extend the loss gradient theorem of~\citet{hazan2010direct} to general non-linear discriminant functions.

%In the following we first illustrate how to directly minimize the task-loss using non-linear and non-convex scoring functions, \eg, composite functions represented by neural networks. To demonstrate applicability of our technique to non-decomposable task-loss functions we then design a general yet efficient dynamic programming approach to optimize the AP loss. Before concluding we demonstrate the performance of our two contributions on a set of experiments involving both synthetic and real-world data.
